A System for Morphology-Task Generalization via Unified Representation and Behavior Distillation

The rise of generalist large-scale models in natural language and vision has made us expect that a massive data-driven approach could achieve broader generalization in other domains such as continuous control. In this work, we explore a method for learning a single policy that manipulates various forms of agents to solve various tasks by distilling a large amount of proficient behavioral data. In order to align input-output (IO) interface among multiple tasks and diverse agent morphologies while preserving essential 3D geometric relations, we introduce morphology-task graph, which treats observations, actions and goals/task in a unified graph representation. We also develop MxT-Bench for fast large-scale behavior generation, which supports procedural generation of diverse morphology-task combinations with a minimal blueprint and hardware-accelerated simulator. Through efficient representation and architecture selection on MxT-Bench, we find out that a morphology-task graph representation coupled with Transformer architecture improves the multi-task performances compared to other baselines including recent discrete tokenization, and provides better prior knowledge for zero-shot transfer or sample efficiency in downstream multi-task imitation learning. Our work suggests large diverse offline datasets, unified IO representation, and policy representation and architecture selection through supervised learning form a promising approach for studying and advancing morphology-task generalization.

==> _old/experiment_summary.tex <==
\section{Additional Results}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.7}{
\begin{tabular}{lcccccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6  \\
\midrule
MLP & 13.55 $\pm$ 5.35 & 43.80 $\pm$ 17.11 & 22.18 $\pm$ 13.02 & 11.31 $\pm$ 13.90 & 23.90 $\pm$ 3.66 & 44.94 $\pm$ 7.09 & 26.19 $\pm$ 5.06 & 28.29 $\pm$ 9.90 \\
AM & 85.23 $\pm$ 4.28 & 96.67 $\pm$ 0.76 & 88.46 $\pm$ 1.42 & 74.52 $\pm$ 3.42 & 25.66 $\pm$ 12.76 & 28.51 $\pm$ 7.61 & 48.54 $\pm$ 17.92 & 34.93 $\pm$ 7.03 \\
AM - id & 90.05 $\pm$ 3.51 & 96.81 $\pm$ 2.36 & 92.79 $\pm$ 3.28 & 89.98 $\pm$ 2.70 & 41.72 $\pm$ 7.89 & 64.41 $\pm$ 4.63 & 66.13 $\pm$ 12.60 & 55.20 $\pm$ 7.88 \\
MM - m - jv - rp & 88.03 $\pm$ 2.76 & 95.63 $\pm$ 1.19 & 91.09 $\pm$ 3.16 & 91.42 $\pm$ 1.64 & 44.12 $\pm$ 11.58 & 63.05 $\pm$ 2.79 & 74.63 $\pm$ 3.36 & 52.71 $\pm$ 19.30  \\
MM - m - jv - rr & 91.75 $\pm$ 1.79 & 97.95 $\pm$ 1.21 & 94.83 $\pm$ 2.86 & 90.52 $\pm$ 2.07 & 55.91 $\pm$ 6.04 & 69.01 $\pm$ 4.72 & 77.72 $\pm$ 3.02 & 61.98 $\pm$ 8.21  \\
MM - m - jv & 87.67 $\pm$ 2.66 & 94.42 $\pm$ 1.37 & 91.49 $\pm$ 2.54 & 92.40 $\pm$ 0.43 & 50.63 $\pm$ 3.44 & 64.42 $\pm$ 7.16 & 77.75 $\pm$ 8.42 & 60.46 $\pm$ 20.87  \\
MM - m & 89.71 $\pm$ 2.63 & 95.90 $\pm$ 0.87 & 92.67 $\pm$ 1.76 & 92.18 $\pm$ 2.29 & 53.34 $\pm$ 3.86 & 65.40 $\pm$ 8.52 & 78.45 $\pm$ 3.49 & 65.90 $\pm$ 2.00 \\
MM & 83.49 $\pm$ 7.48 & 96.52 $\pm$ 1.63 & 92.18 $\pm$ 1.04 & 90.92 $\pm$ 2.81 & 65.19 $\pm$ 12.81 & 78.08 $\pm$ 8.71 & 78.71 $\pm$ 6.07 & 57.65 $\pm$ 7.84  \\
\midrule
 & centipede\_7 & worm\_3 & worm\_4 & worm\_5 & worm\_6 & worm\_7 & \multicolumn{2}{c}{\textbf{Average}}\\
\midrule
MLP & 44.30 $\pm$ 11.93 & 0.00 $\pm$ 0.00 & 6.60 $\pm$ 8.05 & 5.23 $\pm$ 8.61 & 18.39 $\pm$ 6.08 & 28.90 $\pm$ 14.19 & \multicolumn{2}{c}{ 22.68 \% } \\
AM & 4.25 $\pm$ 2.68 & 20.39 $\pm$ 16.21 & 37.66 $\pm$ 10.48 & 24.68 $\pm$ 6.76 & 26.70 $\pm$ 10.51 & 20.13 $\pm$ 10.83 &  \multicolumn{2}{c}{ 44.02 \% } \\
AM - id & 6.11 $\pm$ 6.22 & 25.87 $\pm$ 15.51 & 45.72 $\pm$ 9.89 & 43.71 $\pm$ 12.40 & 21.64 $\pm$ 14.38 & 28.40 $\pm$ 7.02 & \multicolumn{2}{c}{ 54.90 \% } \\
MM - m - jv - rp & 13.92 $\pm$ 4.06 & 24.48 $\pm$ 7.51 & 51.68 $\pm$ 5.53 & 52.79 $\pm$ 6.09 & 26.55 $\pm$ 8.47 & 15.58 $\pm$ 7.68 &  \multicolumn{2}{c}{ 56.12 \% } \\
MM - m - jv - rr & 9.68 $\pm$ 2.32 & 23.10 $\pm$ 10.72 & 53.96 $\pm$ 14.23 & 63.63 $\pm$ 14.58 & 47.26 $\pm$ 13.89 & 34.32 $\pm$ 20.55 & \multicolumn{2}{c}{ 62.26 \% } \\
MM - m - jv & 6.06 $\pm$ 4.34 & 26.13 $\pm$ 2.54 & 47.25 $\pm$ 6.75 & 48.39 $\pm$ 17.57 & 37.85 $\pm$ 10.17 & 22.38 $\pm$ 20.38 & \multicolumn{2}{c}{ 57.67 \% } \\
MM - m & 9.02 $\pm$ 6.41 & 24.14 $\pm$ 5.32 & 50.80 $\pm$ 4.04 & 40.16 $\pm$ 12.47 & 24.92 $\pm$ 4.37 & 20.34 $\pm$ 10.92 & \multicolumn{2}{c}{ 57.35 \% } \\
MM & 13.69 $\pm$ 11.54 & 26.82 $\pm$ 4.64 & 45.13 $\pm$ 12.41 & 39.90 $\pm$ 15.07 & 17.22 $\pm$ 16.51 & 15.00 $\pm$ 13.18 & \multicolumn{2}{c}{ 57.18 \% } \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in acw\_touch (12k).}
\label{tab:acw_touch_obs}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.7}{
\begin{tabular}{lcccccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6  \\
\midrule
MLP & 13.55 $\pm$ 5.35 & 43.80 $\pm$ 17.11 & 22.18 $\pm$ 13.02 & 11.31 $\pm$ 13.90 & 23.90 $\pm$ 3.66 & 44.94 $\pm$ 7.09 & 26.19 $\pm$ 5.06 & 28.29 $\pm$ 9.90 \\
AM & 85.23 $\pm$ 4.28 & 96.67 $\pm$ 0.76 & 88.46 $\pm$ 1.42 & 74.52 $\pm$ 3.42 & 25.66 $\pm$ 12.76 & 28.51 $\pm$ 7.61 & 48.54 $\pm$ 17.92 & 34.93 $\pm$ 7.03 \\
MM & 83.49 $\pm$ 7.48 & 96.52 $\pm$ 1.63 & 92.18 $\pm$ 1.04 & 90.92 $\pm$ 2.81 & 65.19 $\pm$ 12.81 & 78.08 $\pm$ 8.71 & 78.71 $\pm$ 6.07 & 57.65 $\pm$ 7.84  \\
Edge1 & 80.45 $\pm$ 5.94 & 92.14 $\pm$ 3.45 & 75.90 $\pm$ 11.96 & 84.97 $\pm$ 1.79 & 64.27 $\pm$ 3.29 & 73.74 $\pm$ 6.66 & 78.35 $\pm$ 5.42 & 63.80 $\pm$ 11.59 \\
Edge2 & 79.51 $\pm$ 2.98 & 95.25 $\pm$ 1.22 & 80.61 $\pm$ 5.95 & 81.33 $\pm$ 5.34 & 58.92 $\pm$ 15.75 & 79.66 $\pm$ 2.04 & 75.04 $\pm$ 8.01 & 54.50 $\pm$ 17.30 \\
Edge3 & 76.49 $\pm$ 9.98 & 95.25 $\pm$ 2.56 & 73.54 $\pm$ 13.00 & 66.24 $\pm$ 4.58 & 49.81 $\pm$ 13.89 & 65.94 $\pm$ 12.11 & 65.01 $\pm$ 12.84 & 37.34 $\pm$ 12.49 \\
Edge4 & 70.12 $\pm$ 9.97 & 92.77 $\pm$ 3.61 & 71.15 $\pm$ 9.47 & 73.89 $\pm$ 13.40 & 49.89 $\pm$ 16.95 & 59.59 $\pm$ 9.57 & 54.25 $\pm$ 13.53 & 42.59 $\pm$ 14.11 \\
Edge5 & 73.14 $\pm$ 7.96 & 91.17 $\pm$ 1.85 & 72.61 $\pm$ 7.13 & 75.75 $\pm$ 8.04 & 57.61 $\pm$ 8.12 & 60.19 $\pm$ 4.03 & 66.45 $\pm$ 5.61 & 51.82 $\pm$ 14.25 \\
Edge6 & 67.25 $\pm$ 12.34 & 92.71 $\pm$ 2.62 & 80.25 $\pm$ 2.73 & 76.86 $\pm$ 4.33 & 43.69 $\pm$ 17.99 & 68.37 $\pm$ 10.82 & 61.49 $\pm$ 9.54 & 48.63 $\pm$ 20.44 \\
Edge7 & 81.30 $\pm$ 5.84 & 93.13 $\pm$ 1.56 & 80.33 $\pm$ 4.11 & 79.00 $\pm$ 3.82 & 68.53 $\pm$ 4.73 & 77.43 $\pm$ 3.00 & 74.40 $\pm$ 8.71 & 55.79 $\pm$ 3.17 \\
Edge8 & 81.41 $\pm$ 6.36 & 95.40 $\pm$ 1.70 & 79.32 $\pm$ 6.97 & 80.69 $\pm$ 7.41 & 55.94 $\pm$ 15.42 & 76.83 $\pm$ 4.30 & 76.80 $\pm$ 10.17 & 60.39 $\pm$ 9.25 \\
\midrule
 & centipede\_7 & worm\_3 & worm\_4 & worm\_5 & worm\_6 & worm\_7 & \multicolumn{2}{c}{\textbf{Average}}\\
\midrule
MLP & 44.30 $\pm$ 11.93 & 0.00 $\pm$ 0.00 & 6.60 $\pm$ 8.05 & 5.23 $\pm$ 8.61 & 18.39 $\pm$ 6.08 & 28.90 $\pm$ 14.19 & \multicolumn{2}{c}{ 22.68 \% } \\
AM & 4.25 $\pm$ 2.68 & 20.39 $\pm$ 16.21 & 37.66 $\pm$ 10.48 & 24.68 $\pm$ 6.76 & 26.70 $\pm$ 10.51 & 20.13 $\pm$ 10.83 &  \multicolumn{2}{c}{ 44.02 \% } \\
MM & 13.69 $\pm$ 11.54 & 26.82 $\pm$ 4.64 & 45.13 $\pm$ 12.41 & 39.90 $\pm$ 15.07 & 17.22 $\pm$ 16.51 & 15.00 $\pm$ 13.18 & \multicolumn{2}{c}{ 57.18 \% } \\
Edge1 & 27.86 $\pm$ 9.98 & 7.29 $\pm$ 9.85 & 37.48 $\pm$ 10.95 & 47.07 $\pm$ 10.12 & 12.97 $\pm$ 11.41 & 31.88 $\pm$ 21.23 & \multicolumn{2}{c}{ 55.58 \% } \\
Edge2 & 22.51 $\pm$ 6.80 & 0.00 $\pm$ 0.00 & 30.19 $\pm$ 19.83 & 41.81 $\pm$ 20.76 & 21.38 $\pm$ 15.47 & 29.45 $\pm$ 21.00 & \multicolumn{2}{c}{ 53.58 \% }\\
Edge3 & 19.06 $\pm$ 7.40 & 0.00 $\pm$ 0.00 & 32.98 $\pm$ 5.75 & 57.04 $\pm$ 10.02 & 13.77 $\pm$ 7.68 & 26.39 $\pm$ 16.95 & \multicolumn{2}{c}{ 48.49 \% }\\
Edge4 & 29.95 $\pm$ 15.11 & 0.00 $\pm$ 0.00 & 35.14 $\pm$ 12.55 & 54.40 $\pm$ 13.38 & 39.22 $\pm$ 18.76 & 24.56 $\pm$ 10.71 & \multicolumn{2}{c}{49.82 \% } \\
Edge5 & 30.83 $\pm$ 23.67 & 1.31 $\pm$ 2.26 & 36.85 $\pm$ 11.93 & 39.04 $\pm$ 21.38 & 23.97 $\pm$ 14.41 & 20.95 $\pm$ 23.27 & \multicolumn{2}{c}{ 50.12 \% } \\
Edge6 & 23.31 $\pm$ 11.93 & 6.93 $\pm$ 6.06 & 32.48 $\pm$ 23.17 & 59.98 $\pm$ 11.02 & 39.74 $\pm$ 8.83 & 27.34 $\pm$ 17.60 & \multicolumn{2}{c}{ 52.07 \% }\\
Edge7 & 32.21 $\pm$ 19.71 & 3.94 $\pm$ 6.82 & 44.17 $\pm$ 10.74 & 60.28 $\pm$ 15.51 & 31.80 $\pm$ 22.91 & 31.61 $\pm$ 14.69 & \multicolumn{2}{c}{ 58.14 \% }\\
Edge8 & 24.75 $\pm$ 13.82 & 2.81 $\pm$ 2.82 & 37.55 $\pm$ 10.41 & 52.34 $\pm$ 18.98 & 27.16 $\pm$ 14.60 & 49.23 $\pm$ 19.93 & \multicolumn{2}{c}{ 57.19 \% }\\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in acw\_touch (12k).}
\label{tab:acw_touch_edge}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 20.00 $\pm$ 5.10 & 28.07 $\pm$ 8.08 & 23.55 $\pm$ 3.11 & 3.71 $\pm$ 1.28 & 18.83 \% \\
AM & 87.21 $\pm$ 3.59 & 97.65 $\pm$ 2.03 & 96.89 $\pm$ 1.79 & 93.68 $\pm$ 2.39 & 93.86 \% \\
AM - id & 83.75 $\pm$ 4.85 & 98.23 $\pm$ 0.64 & 98.32 $\pm$ 0.31 & 95.72 $\pm$ 2.80 & 94.00 \% \\
MM - m - jv - rp & 76.55 $\pm$ 3.86 & 96.85 $\pm$ 1.25 & 95.49 $\pm$ 0.45 & 94.83 $\pm$ 1.80 & 90.93 \% \\
MM - m - jv - rr & 72.12 $\pm$ 3.38 & 98.07 $\pm$ 0.52 & 97.70 $\pm$ 0.56 & 95.75 $\pm$ 2.10 & 90.91 \% \\
MM - m - jv & 72.17 $\pm$ 4.32 & 96.19 $\pm$ 0.47 & 95.74 $\pm$ 0.78 & 95.82 $\pm$ 0.99 & 89.98 \% \\
MM - m & 66.68 $\pm$ 7.43 & 96.96 $\pm$ 0.51 & 95.99 $\pm$ 2.44 & 94.27 $\pm$ 3.03 & 88.47 \% \\
MM & 66.21 $\pm$ 3.56 & 92.26 $\pm$ 3.08 & 90.34 $\pm$ 3.96 & 77.20 $\pm$ 9.99 & 81.50 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_touch (12k).}
\label{tab:ant_touch_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 20.00 $\pm$ 5.10 & 28.07 $\pm$ 8.08 & 23.55 $\pm$ 3.11 & 3.71 $\pm$ 1.28 & 18.83 \% \\
AM & 87.21 $\pm$ 3.59 & 97.65 $\pm$ 2.03 & 96.89 $\pm$ 1.79 & 93.68 $\pm$ 2.39 & 93.86 \% \\
MM & 66.21 $\pm$ 3.56 & 92.26 $\pm$ 3.08 & 90.34 $\pm$ 3.96 & 77.20 $\pm$ 9.99 & 81.50 \%
\\
Edge1 & 51.57 $\pm$ 16.81 & 81.47 $\pm$ 10.24 & 53.86 $\pm$ 24.65 & 45.06 $\pm$ 18.18 & 57.99 \% \\
Edge2 & 37.78 $\pm$ 13.84 & 56.80 $\pm$ 7.90 & 40.22 $\pm$ 11.04 & 24.11 $\pm$ 7.27 & 39.73 \% \\
Edge3 & 64.31 $\pm$ 8.29 & 82.95 $\pm$ 6.53 & 52.51 $\pm$ 16.51 & 30.76 $\pm$ 18.85 & 57.63 \% \\
Edge4 & 44.39 $\pm$ 16.42 & 75.10 $\pm$ 22.20 & 67.36 $\pm$ 13.79 & 56.24 $\pm$ 10.26 & 60.77 \% \\
Edge5 & 42.53 $\pm$ 14.46 & 62.99 $\pm$ 23.45 & 42.21 $\pm$ 19.43 & 27.63 $\pm$ 12.61 & 43.84 \% \\
Edge6 & 29.85 $\pm$ 12.20 & 63.26 $\pm$ 13.32 & 36.96 $\pm$ 9.59 & 34.49 $\pm$ 5.74 & 41.14 \% \\
Edge7 & 50.23 $\pm$ 15.58 & 64.94 $\pm$ 10.96 & 39.77 $\pm$ 14.14 & 24.95 $\pm$ 10.39 & 44.97 \% \\
Edge8 & 51.97 $\pm$ 15.23 & 86.60 $\pm$ 11.12 & 61.61 $\pm$ 22.21 & 43.23 $\pm$ 32.35 & 60.85 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_touch (12k).}
\label{tab:ant_touch_edge}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{1.0}{
\begin{tabular}{lcccc}
\toprule
 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 0.76 $\pm$ 1.32 & 1.75 $\pm$ 1.01 & 1.95 $\pm$ 0.87 & 1.49 \% \\
AM & 2.88 $\pm$ 1.94 & 16.28 $\pm$ 13.43 & 10.44 $\pm$ 3.33 & 9.86 \% \\
AM - id & 3.48 $\pm$ 1.15 & 17.65 $\pm$ 15.81 & 38.04 $\pm$ 19.39 & 19.72 \% \\
MM - m - jv - rp & 3.20 $\pm$ 2.73 & 19.95 $\pm$ 13.91 & 27.37 $\pm$ 22.94 & 16.84 \% \\
MM - m - jv - rr & 5.59 $\pm$ 2.82 & 15.04 $\pm$ 12.51 & 7.18 $\pm$ 6.81 & 9.27 \% \\
MM - m - jv & 10.11 $\pm$ 8.90 & 19.31 $\pm$ 17.87 & 23.16 $\pm$ 13.73 & 17.53 \% \\
MM - m & 13.89 $\pm$ 17.56 & 24.24 $\pm$ 13.37 & 23.31 $\pm$ 16.84 & 20.48 \% \\
MM & 2.33 $\pm$ 0.76 & 14.81 $\pm$ 17.24 & 9.48 $\pm$ 5.81 & 8.87 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_c (12k).}
% ant\_reach2\_handsup
\label{tab:ant_reach2_handsup}
% \vskip -0.1in
\end{table*}



\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.9}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & centipede\_3  \\
\midrule
MLP & 19.01 $\pm$ 13.93 & 50.15 $\pm$ 7.39 & 14.06 $\pm$ 12.81 & 6.87 $\pm$ 5.88 & 23.05 $\pm$ 8.32 \\
AM & 92.52 $\pm$ 2.85 & 98.65 $\pm$ 0.40 & 91.72 $\pm$ 4.20 & 81.08 $\pm$ 1.84 & 29.09 $\pm$ 4.27  \\
AM - id  & 93.72 $\pm$ 1.07 & 97.86 $\pm$ 0.95 & 94.78 $\pm$ 1.53 & 92.22 $\pm$ 1.54 & 50.08 $\pm$ 9.81 \\
MM - m - jv - rp & 91.14 $\pm$ 1.70 & 96.09 $\pm$ 1.87 & 94.07 $\pm$ 0.71 & 91.67 $\pm$ 2.34 & 46.36 $\pm$ 10.95 \\
MM - m - jv - rr & 92.32 $\pm$ 2.64 & 98.31 $\pm$ 0.58 & 96.67 $\pm$ 1.99 & 94.24 $\pm$ 1.24 & 60.09 $\pm$ 5.88 \\
MM - m - jv & 93.61 $\pm$ 1.83 & 97.15 $\pm$ 0.81 & 94.72 $\pm$ 0.87 & 92.06 $\pm$ 2.80 & 62.16 $\pm$ 8.60  \\
MM - m & 90.87 $\pm$ 1.86 & 96.01 $\pm$ 1.21 & 93.18 $\pm$ 2.61 & 90.32 $\pm$ 4.11 & 55.80 $\pm$ 10.15 \\
MM & 75.13 $\pm$ 16.52 & 93.63 $\pm$ 1.47 & 78.48 $\pm$ 9.28 & 79.53 $\pm$ 7.93 & 65.69 $\pm$ 6.61 \\
\midrule
 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average} \\
\midrule
MLP & 31.60 $\pm$ 8.78 & 40.42 $\pm$ 4.38 & 30.37 $\pm$ 7.20 & 48.68 $\pm$ 5.62 & 29.36 \% \\
AM & 49.54 $\pm$ 8.03 & 58.29 $\pm$ 9.39 & 47.98 $\pm$ 10.60 & 10.21 $\pm$ 3.63 & 62.12 \% \\
AM - id & 71.85 $\pm$ 3.40 & 72.90 $\pm$ 2.06 & 59.35 $\pm$ 12.10 & 22.32 $\pm$ 13.85 & 72.79 \% \\
MM - m - jv - rp & 72.69 $\pm$ 3.27 & 74.28 $\pm$ 9.15 & 59.62 $\pm$ 8.07 & 13.83 $\pm$ 4.85 & 71.08 \% \\
MM - m - jv - rr & 73.43 $\pm$ 2.96 & 83.17 $\pm$ 2.45 & 72.69 $\pm$ 2.40 & 28.47 $\pm$ 18.54 & 77.71 \% \\
MM - m - jv & 70.46 $\pm$ 7.78 & 78.79 $\pm$ 2.98 & 70.59 $\pm$ 6.67 & 21.40 $\pm$ 12.19 & 75.66 \% \\
MM - m & 77.28 $\pm$ 4.74 & 81.80 $\pm$ 1.10 & 67.19 $\pm$ 8.13 & 17.30 $\pm$ 13.32 & 74.42 \% \\
MM & 77.65 $\pm$ 11.48 & 68.96 $\pm$ 1.63 & 61.11 $\pm$ 3.16 & 18.43 $\pm$ 17.41 & 68.73 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in acw\_touch (12k).}
\label{tab:ac_touch_obs}
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.9}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & centipede\_3  \\
\midrule
MLP & 19.01 $\pm$ 13.93 & 50.15 $\pm$ 7.39 & 14.06 $\pm$ 12.81 & 6.87 $\pm$ 5.88 & 23.05 $\pm$ 8.32 \\
AM & 92.52 $\pm$ 2.85 & 98.65 $\pm$ 0.40 & 91.72 $\pm$ 4.20 & 81.08 $\pm$ 1.84 & 29.09 $\pm$ 4.27  \\
MM & 75.13 $\pm$ 16.52 & 93.63 $\pm$ 1.47 & 78.48 $\pm$ 9.28 & 79.53 $\pm$ 7.93 & 65.69 $\pm$ 6.61 \\
Edge1 & 84.24 $\pm$ 6.72 & 94.67 $\pm$ 2.98 & 83.10 $\pm$ 7.43 & 81.07 $\pm$ 4.07 & 69.79 $\pm$ 9.84 \\
Edge2 & 80.51 $\pm$ 6.02 & 93.43 $\pm$ 2.55 & 83.75 $\pm$ 5.76 & 83.22 $\pm$ 4.57 & 56.65 $\pm$ 10.91 \\
Edge3 & 86.88 $\pm$ 3.57 & 95.13 $\pm$ 1.34 & 82.72 $\pm$ 3.78 & 79.27 $\pm$ 4.70 & 67.47 $\pm$ 8.52 \\
Edge4 & 83.64 $\pm$ 2.85 & 92.56 $\pm$ 5.10 & 82.08 $\pm$ 7.33 & 80.68 $\pm$ 4.83 & 52.38 $\pm$ 9.12 \\
Edge5 & 83.91 $\pm$ 4.18 & 96.13 $\pm$ 0.89 & 86.41 $\pm$ 2.25 & 81.98 $\pm$ 3.23 & 68.98 $\pm$ 6.89 \\
Edge6 & 71.83 $\pm$ 6.69 & 93.70 $\pm$ 1.79 & 80.09 $\pm$ 4.76 & 68.90 $\pm$ 15.92 & 55.39 $\pm$ 14.86 \\
Edge7 & 86.70 $\pm$ 4.89 & 95.26 $\pm$ 2.36 & 87.62 $\pm$ 4.70 & 82.37 $\pm$ 8.05 & 67.91 $\pm$ 10.45 \\
Edge8 & 77.24 $\pm$ 5.47 & 95.18 $\pm$ 1.26 & 83.04 $\pm$ 5.14 & 74.98 $\pm$ 4.71 & 59.37 $\pm$ 7.50 \\
\midrule
 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average} \\
\midrule
MLP & 31.60 $\pm$ 8.78 & 40.42 $\pm$ 4.38 & 30.37 $\pm$ 7.20 & 48.68 $\pm$ 5.62 & 29.36 \% \\
AM & 49.54 $\pm$ 8.03 & 58.29 $\pm$ 9.39 & 47.98 $\pm$ 10.60 & 10.21 $\pm$ 3.63 & 62.12 \% \\
MM & 77.65 $\pm$ 11.48 & 68.96 $\pm$ 1.63 & 61.11 $\pm$ 3.16 & 18.43 $\pm$ 17.41 & 68.73 \% \\
Edge1 & 80.50 $\pm$ 7.07 & 71.59 $\pm$ 7.13 & 58.71 $\pm$ 9.10 & 47.29 $\pm$ 11.18 & 74.55 \% \\
Edge2 & 76.03 $\pm$ 5.22 & 74.23 $\pm$ 5.34 & 58.01 $\pm$ 11.15 & 51.66 $\pm$ 12.37 & 73.05 \% \\
Edge3 & 77.62 $\pm$ 5.96 & 68.53 $\pm$ 13.98 & 61.10 $\pm$ 11.98 & 46.53 $\pm$ 13.98 & 73.92 \% \\
Edge4 & 76.27 $\pm$ 8.21 & 71.74 $\pm$ 7.03 & 67.07 $\pm$ 10.25 & 46.52 $\pm$ 12.81 & 72.55 \% \\
Edge5 & 78.26 $\pm$ 4.32 & 76.94 $\pm$ 7.10 & 59.01 $\pm$ 13.85 & 39.50 $\pm$ 14.90 & 74.57 \% \\
Edge6 & 76.78 $\pm$ 5.48 & 70.02 $\pm$ 7.49 & 48.48 $\pm$ 22.34 & 34.68 $\pm$ 9.90 & 66.65 \% \\
Edge7 & 73.91 $\pm$ 13.99 & 75.73 $\pm$ 6.27 & 64.35 $\pm$ 15.13 & 46.56 $\pm$ 15.35 & 75.60 \% \\
Edge8 & 78.70 $\pm$ 7.65 & 74.55 $\pm$ 6.70 & 53.21 $\pm$ 13.76 & 35.56 $\pm$ 15.88 & 70.20 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in acw\_touch (12k).}
\label{tab:ac_touch_edge}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average}  \\
\midrule
MLP & 22.14 $\pm$ 10.59 & 41.98 $\pm$ 3.89 & 40.01 $\pm$ 3.51 & 39.36 $\pm$ 9.45 & 55.60 $\pm$ 3.04 & 39.82 \% \\
AM& 56.73 $\pm$ 12.77 & 77.83 $\pm$ 6.01 & 82.12 $\pm$ 1.83 & 73.48 $\pm$ 9.27 & 23.91 $\pm$ 18.95 & 62.81 \% \\
AM - id  & 66.45 $\pm$ 5.66 & 86.15 $\pm$ 1.57 & 88.94 $\pm$ 3.15 & 78.63 $\pm$ 5.48 & 38.97 $\pm$ 12.20 & 71.83 \% \\
MM - m - jv - rp & 61.08 $\pm$ 11.23 & 84.73 $\pm$ 5.28 & 88.55 $\pm$ 6.17 & 81.60 $\pm$ 7.71 & 45.48 $\pm$ 10.33 & 72.29 \% \\
MM - m - jv - rr & 70.31 $\pm$ 6.99 & 85.21 $\pm$ 4.26 & 87.36 $\pm$ 3.04 & 78.32 $\pm$ 3.87 & 40.52 $\pm$ 8.30 & 72.34 \% \\
MM - m - jv & 66.90 $\pm$ 8.10 & 82.71 $\pm$ 5.28 & 88.29 $\pm$ 4.19 & 81.53 $\pm$ 2.38 & 48.14 $\pm$ 7.00 & 73.51 \% \\
MM - m & 59.57 $\pm$ 13.55 & 82.31 $\pm$ 6.79 & 87.12 $\pm$ 3.63 & 85.12 $\pm$ 3.19 & 55.60 $\pm$ 8.21 & 73.94 \% \\
MM & 78.28 $\pm$ 5.54 & 90.15 $\pm$ 2.07 & 88.45 $\pm$ 2.17 & 80.86 $\pm$ 4.97 & 42.36 $\pm$ 15.78 & 76.02 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in centipede\_touch (12k).}
\label{tab:centipede_touch_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average}  \\
\midrule
MLP & 22.14 $\pm$ 10.59 & 41.98 $\pm$ 3.89 & 40.01 $\pm$ 3.51 & 39.36 $\pm$ 9.45 & 55.60 $\pm$ 3.04 & 39.82 \% \\
AM& 56.73 $\pm$ 12.77 & 77.83 $\pm$ 6.01 & 82.12 $\pm$ 1.83 & 73.48 $\pm$ 9.27 & 23.91 $\pm$ 18.95 & 62.81 \% \\
MM & 78.28 $\pm$ 5.54 & 90.15 $\pm$ 2.07 & 88.45 $\pm$ 2.17 & 80.86 $\pm$ 4.97 & 42.36 $\pm$ 15.78 & 76.02 \% \\
Edge1 & 62.39 $\pm$ 7.77 & 83.33 $\pm$ 2.80 & 77.10 $\pm$ 3.71 & 61.35 $\pm$ 15.30 & 62.15 $\pm$ 9.99 & 69.26 \% \\
Edge2 & 49.04 $\pm$ 5.04 & 81.98 $\pm$ 8.66 & 71.62 $\pm$ 17.01 & 59.72 $\pm$ 13.51 & 60.40 $\pm$ 9.28 & 64.55 \% \\
Edge3 & 62.72 $\pm$ 14.70 & 78.06 $\pm$ 8.62 & 81.66 $\pm$ 3.96 & 68.53 $\pm$ 12.83 & 48.97 $\pm$ 23.25 & 67.99 \% \\
Edge4 & 57.11 $\pm$ 8.17 & 84.84 $\pm$ 5.78 & 80.51 $\pm$ 7.01 & 72.57 $\pm$ 7.57 & 52.96 $\pm$ 24.11 & 69.60 \% \\
Edge5 & 58.40 $\pm$ 11.76 & 70.77 $\pm$ 15.19 & 71.24 $\pm$ 13.08 & 59.20 $\pm$ 18.01 & 68.42 $\pm$ 7.52 & 65.61 \% \\
Edge6 & 33.29 $\pm$ 19.59 & 72.71 $\pm$ 10.15 & 65.58 $\pm$ 23.02 & 51.42 $\pm$ 18.63 & 57.80 $\pm$ 18.04 & 56.16 \% \\
Edge7 & 69.25 $\pm$ 5.89 & 87.91 $\pm$ 3.00 & 79.13 $\pm$ 3.22 & 78.69 $\pm$ 6.98 & 68.05 $\pm$ 6.86 & 76.61 \% \\
Edge8 & 68.76 $\pm$ 6.25 & 88.82 $\pm$ 1.50 & 86.09 $\pm$ 3.89 & 76.06 $\pm$ 9.58 & 60.65 $\pm$ 10.06 & 76.07 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in centipede\_touch (12k).}
\label{tab:centipede_touch_edge}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & worm\_3 & worm\_4 & worm\_5 & worm\_6 & worm\_7 & \textbf{Average}  \\
\midrule
MLP & 4.65 $\pm$ 2.98 & 41.78 $\pm$ 8.44 & 47.36 $\pm$ 7.29 & 38.92 $\pm$ 15.05 & 22.44 $\pm$ 10.15 & 31.03 \% \\
AM & 29.93 $\pm$ 4.59 & 58.07 $\pm$ 5.91 & 57.74 $\pm$ 12.37 & 48.22 $\pm$ 9.36 & 44.55 $\pm$ 2.98 & 47.70 \% \\
AM - id & 41.46 $\pm$ 12.40 & 66.05 $\pm$ 11.60 & 59.37 $\pm$ 8.37 & 44.23 $\pm$ 8.94 & 37.50 $\pm$ 10.64 & 49.72 \% \\
MM - m - jv - rp & 37.54 $\pm$ 6.97 & 64.71 $\pm$ 7.17 & 64.55 $\pm$ 8.45 & 44.59 $\pm$ 18.04 & 41.75 $\pm$ 18.00 & 50.63 \% \\
MM - m - jv - rr & 30.52 $\pm$ 6.67 & 68.40 $\pm$ 4.24 & 58.49 $\pm$ 3.48 & 56.52 $\pm$ 1.41 & 38.00 $\pm$ 13.53 & 50.39 \% \\
MM - m - jv & 37.72 $\pm$ 9.05 & 70.62 $\pm$ 6.94 & 66.71 $\pm$ 10.79 & 57.47 $\pm$ 5.71 & 41.33 $\pm$ 6.37 & 54.77 \% \\
MM - m & 36.65 $\pm$ 5.18 & 43.56 $\pm$ 17.15 & 56.91 $\pm$ 9.52 & 31.47 $\pm$ 10.88 & 18.25 $\pm$ 10.26 & 37.37 \% \\
MM & 45.98 $\pm$ 10.33 & 65.61 $\pm$ 13.10 & 57.11 $\pm$ 8.56 & 40.53 $\pm$ 21.14 & 37.26 $\pm$ 23.24 & 49.30 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in worm\_touch (12k).}
\label{tab:worm_touch_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & ant\_2 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 0.76 $\pm$ 1.32 & 13.95 $\pm$ 9.28 & 10.37 $\pm$ 7.82 & 17.72 $\pm$ 5.81 & 26.84 $\pm$ 9.72 & 13.93 \% \\
AM & 4.99 $\pm$ 3.60 & 68.81 $\pm$ 2.99 & 83.88 $\pm$ 4.07 & 93.51 $\pm$ 2.46 & 96.62 $\pm$ 1.86 & 69.56 \% \\
AM - id & 9.24 $\pm$ 8.19 & 66.62 $\pm$ 7.22 & 82.43 $\pm$ 9.46 & 92.67 $\pm$ 2.70 & 95.66 $\pm$ 1.78 & 69.32 \% \\
MM - m - jv - rp & 5.02 $\pm$ 2.56 & 68.13 $\pm$ 6.42 & 79.47 $\pm$ 6.90 & 89.23 $\pm$ 6.88 & 92.81 $\pm$ 5.00 & 66.93 \% \\
MM - m - jv - rr & 3.15 $\pm$ 2.83 & 69.21 $\pm$ 3.65 & 86.60 $\pm$ 2.56 & 94.57 $\pm$ 2.47 & 97.37 $\pm$ 1.76 & 70.18 \% \\
MM - m - jv & 0.97 $\pm$ 1.00 & 75.65 $\pm$ 2.72 & 83.10 $\pm$ 3.76 & 94.58 $\pm$ 1.74 & 95.26 $\pm$ 1.92 & 69.91 \% \\
MM - m & 6.36 $\pm$ 5.44 & 63.99 $\pm$ 1.93 & 88.69 $\pm$ 4.07 & 93.66 $\pm$ 2.60 & 98.14 $\pm$ 0.65 & 70.17 \% \\
MM & 2.08 $\pm$ 2.44 & 66.74 $\pm$ 6.56 & 75.74 $\pm$ 7.19 & 88.54 $\pm$ 5.46 & 94.24 $\pm$ 2.98 & 65.47 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_reach\_hard (12k).}
\label{tab:ant_reach_hard_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & ant\_2 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 0.76 $\pm$ 1.32 & 13.95 $\pm$ 9.28 & 10.37 $\pm$ 7.82 & 17.72 $\pm$ 5.81 & 26.84 $\pm$ 9.72 & 13.93 \% \\
AM & 4.99 $\pm$ 3.60 & 68.81 $\pm$ 2.99 & 83.88 $\pm$ 4.07 & 93.51 $\pm$ 2.46 & 96.62 $\pm$ 1.86 & 69.56 \% \\
MM & 2.08 $\pm$ 2.44 & 66.74 $\pm$ 6.56 & 75.74 $\pm$ 7.19 & 88.54 $\pm$ 5.46 & 94.24 $\pm$ 2.98 & 65.47 \% \\
Edge1 & 6.32 $\pm$ 4.52 & 52.89 $\pm$ 6.63 & 56.42 $\pm$ 2.31 & 83.40 $\pm$ 4.34 & 91.49 $\pm$ 3.64 & 58.10 \% \\
Edge2 & 0.78 $\pm$ 0.95 & 55.24 $\pm$ 9.55 & 69.23 $\pm$ 6.09 & 78.00 $\pm$ 7.74 & 90.48 $\pm$ 6.64 & 58.75 \% \\
Edge3 & 6.52 $\pm$ 5.21 & 54.29 $\pm$ 16.17 & 52.20 $\pm$ 6.65 & 77.29 $\pm$ 5.67 & 87.47 $\pm$ 4.97 & 55.55 \% \\
Edge4 & 2.02 $\pm$ 3.06 & 63.19 $\pm$ 8.45 & 65.53 $\pm$ 3.40 & 76.14 $\pm$ 6.81 & 88.26 $\pm$ 5.40 & 59.03 \% \\
Edge5 & 9.75 $\pm$ 12.59 & 46.02 $\pm$ 10.43 & 72.44 $\pm$ 7.56 & 76.86 $\pm$ 8.29 & 90.08 $\pm$ 3.15 & 59.03 \% \\
Edge6 & 14.17 $\pm$ 13.30 & 50.74 $\pm$ 15.77 & 64.54 $\pm$ 4.30 & 81.88 $\pm$ 8.00 & 89.23 $\pm$ 5.10 & 60.11 \% \\
Edge7 & 1.91 $\pm$ 1.73 & 56.33 $\pm$ 7.85 & 68.69 $\pm$ 10.52 & 77.91 $\pm$ 4.95 & 92.21 $\pm$ 3.28 & 59.41 \% \\
Edge8 & 14.32 $\pm$ 4.27 & 57.43 $\pm$ 9.15 & 67.70 $\pm$ 9.10 & 86.43 $\pm$ 4.95 & 94.06 $\pm$ 2.33 & 63.99 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_reach\_hard (12k).}
\label{tab:ant_reach_hard_edge}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.7}{
\begin{tabular}{lcccccccc}
\toprule
 & ant\_2\_a & ant\_3\_a & ant\_4\_a & ant\_5\_a & ant\_6\_a & ant\_3\_b & ant\_4\_b & ant\_5\_b  \\
\midrule
MLP & 59.60 $\pm$ 6.80 & 52.54 $\pm$ 4.70 & 37.69 $\pm$ 15.92 & 39.30 $\pm$ 19.76 & 13.87 $\pm$ 13.36 & 9.59 $\pm$ 7.58 & 3.40 $\pm$ 5.89 & 0.20 $\pm$ 0.34 \\
AM & 67.48 $\pm$ 10.98 & 86.33 $\pm$ 2.22 & 76.44 $\pm$ 5.66 & 91.68 $\pm$ 2.45 & 84.24 $\pm$ 7.06 & 87.14 $\pm$ 7.33 & 74.16 $\pm$ 8.63 & 87.58 $\pm$ 4.68 \\
AM - id & 70.51 $\pm$ 6.61 & 85.99 $\pm$ 4.02 & 75.61 $\pm$ 4.26 & 96.04 $\pm$ 0.54 & 96.03 $\pm$ 0.91 & 95.90 $\pm$ 1.80 & 82.07 $\pm$ 5.71 & 89.95 $\pm$ 1.93 \\
MM - m - jv - rp & 64.77 $\pm$ 7.07 & 91.29 $\pm$ 1.05 & 78.74 $\pm$ 7.43 & 95.47 $\pm$ 0.40 & 95.34 $\pm$ 0.73 & 3.57 $\pm$ 3.05 & 0.58 $\pm$ 1.01 & 3.60 $\pm$ 6.23 \\
MM - m - jv - rr & 66.07 $\pm$ 4.82 & 82.85 $\pm$ 9.91 & 70.70 $\pm$ 15.99 & 93.46 $\pm$ 2.34 & 92.29 $\pm$ 5.63 & 7.48 $\pm$ 3.53 & 9.11 $\pm$ 13.55 & 18.13 $\pm$ 22.93 \\
MM - m - jv & 66.31 $\pm$ 10.08 & 93.74 $\pm$ 0.45 & 86.15 $\pm$ 4.46 & 96.72 $\pm$ 0.96 & 95.92 $\pm$ 0.71 & 7.02 $\pm$ 5.65 & 12.46 $\pm$ 12.68 & 18.64 $\pm$ 21.95 \\
MM - m & 67.64 $\pm$ 12.76 & 90.22 $\pm$ 3.07 & 81.37 $\pm$ 5.71 & 94.13 $\pm$ 2.51 & 93.65 $\pm$ 1.24 & 2.08 $\pm$ 3.16 & 0.20 $\pm$ 0.34 & 0.58 $\pm$ 0.64 \\
MM & 63.53 $\pm$ 8.21 & 80.02 $\pm$ 6.98 & 80.12 $\pm$ 2.68 & 94.96 $\pm$ 0.95 & 94.71 $\pm$ 1.36 & 0.39 $\pm$ 0.39 & 0.20 $\pm$ 0.34 & 6.79 $\pm$ 10.86 \\
\midrule
 & ant\_6\_b & ant\_4\_c & ant\_5\_c & ant\_6\_c & ant\_4\_d & ant\_5\_d & ant\_6\_d & \textbf{Average}\\
\midrule
MLP & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.76 $\pm$ 1.32 & 0.00 $\pm$ 0.00 & 0.20 $\pm$ 0.34 & 4.31 $\pm$ 7.02 & 0.78 $\pm$ 0.00 & 14.82 \% \\
AM  & 42.83 $\pm$ 21.22 & 4.78 $\pm$ 8.27 & 31.53 $\pm$ 15.00 & 11.01 $\pm$ 18.61 & 42.73 $\pm$ 11.70 & 45.57 $\pm$ 12.87 & 49.56 $\pm$ 9.27 & 58.87 \% \\
AM - id  & 80.43 $\pm$ 3.44 & 13.29 $\pm$ 14.45 & 31.73 $\pm$ 5.41 & 35.50 $\pm$ 12.87 & 39.08 $\pm$ 16.65 & 46.22 $\pm$ 6.24 & 53.87 $\pm$ 5.92 & 66.15 \% \\
MM - m - jv - rp & 0.00 $\pm$ 0.00 & 11.71 $\pm$ 10.11 & 32.29 $\pm$ 22.19 & 25.31 $\pm$ 9.84 & 17.56 $\pm$ 8.29 & 32.10 $\pm$ 19.61 & 51.79 $\pm$ 11.92 & 40.27 \% \\
MM - m - jv - rr & 18.09 $\pm$ 18.20 & 7.26 $\pm$ 12.58 & 33.00 $\pm$ 15.18 & 31.54 $\pm$ 16.04 & 39.47 $\pm$ 14.35 & 54.80 $\pm$ 26.79 & 43.30 $\pm$ 26.04 & 44.50 \% \\
MM - m - jv  & 0.00 $\pm$ 0.00 & 5.47 $\pm$ 9.47 & 30.98 $\pm$ 25.67 & 35.79 $\pm$ 8.02 & 23.87 $\pm$ 12.61 & 49.02 $\pm$ 14.68 & 53.83 $\pm$ 19.46 & 45.06 \% \\
MM - m & 0.00 $\pm$ 0.00 & 24.06 $\pm$ 13.81 & 18.47 $\pm$ 19.76 & 34.01 $\pm$ 9.62 & 34.34 $\pm$ 23.37 & 64.34 $\pm$ 12.38 & 52.32 $\pm$ 9.96 & 43.83 \% \\
MM & 0.20 $\pm$ 0.34 & 11.80 $\pm$ 14.72 & 35.06 $\pm$ 21.47 & 41.31 $\pm$ 15.08 & 1.82 $\pm$ 3.16 & 7.51 $\pm$ 7.69 & 10.65 $\pm$ 8.91 & 35.27 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in ant\_twisters (12k). (a) reach\_handsup, (b) reach\_handsup2, (c) reach2\_handsup, (d) touch\_handsup}
\label{tab:ant_twisters_obs}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.7}{
\begin{tabular}{lcccccccc}
\toprule
 & ant\_2\_a & ant\_3\_a & ant\_4\_a & ant\_5\_a & ant\_6\_a & ant\_3\_b & ant\_4\_b & ant\_5\_b  \\
\midrule
MLP & 59.60 $\pm$ 6.80 & 52.54 $\pm$ 4.70 & 37.69 $\pm$ 15.92 & 39.30 $\pm$ 19.76 & 13.87 $\pm$ 13.36 & 9.59 $\pm$ 7.58 & 3.40 $\pm$ 5.89 & 0.20 $\pm$ 0.34 \\
AM & 67.48 $\pm$ 10.98 & 86.33 $\pm$ 2.22 & 76.44 $\pm$ 5.66 & 91.68 $\pm$ 2.45 & 84.24 $\pm$ 7.06 & 87.14 $\pm$ 7.33 & 74.16 $\pm$ 8.63 & 87.58 $\pm$ 4.68 \\
MM & 63.53 $\pm$ 8.21 & 80.02 $\pm$ 6.98 & 80.12 $\pm$ 2.68 & 94.96 $\pm$ 0.95 & 94.71 $\pm$ 1.36 & 0.39 $\pm$ 0.39 & 0.20 $\pm$ 0.34 & 6.79 $\pm$ 10.86 \\
Edge1 & 73.01 $\pm$ 3.08 & 85.99 $\pm$ 3.89 & 70.10 $\pm$ 13.54 & 90.91 $\pm$ 2.24 & 94.39 $\pm$ 1.16 & 35.81 $\pm$ 31.38 & 4.33 $\pm$ 7.51 & 56.83 $\pm$ 19.77 \\
Edge2 & 75.12 $\pm$ 3.61 & 90.97 $\pm$ 1.46 & 76.14 $\pm$ 13.97 & 92.33 $\pm$ 3.00 & 94.02 $\pm$ 2.01 & 9.28 $\pm$ 8.52 & 2.70 $\pm$ 1.76 & 44.24 $\pm$ 30.68 \\
Edge3 & 65.45 $\pm$ 5.19 & 84.96 $\pm$ 7.90 & 80.53 $\pm$ 2.51 & 91.94 $\pm$ 1.47 & 95.33 $\pm$ 1.35 & 22.57 $\pm$ 19.79 & 1.14 $\pm$ 1.56 & 35.89 $\pm$ 35.91 \\
Edge4 & 65.99 $\pm$ 8.10 & 84.93 $\pm$ 2.30 & 78.97 $\pm$ 6.00 & 83.72 $\pm$ 12.03 & 93.57 $\pm$ 3.31 & 25.67 $\pm$ 18.81 & 19.65 $\pm$ 13.37 & 73.07 $\pm$ 6.56 \\
Edge5 & 74.20 $\pm$ 9.06 & 84.68 $\pm$ 7.04 & 76.50 $\pm$ 3.88 & 92.18 $\pm$ 3.05 & 95.49 $\pm$ 2.52 & 27.21 $\pm$ 26.40 & 9.27 $\pm$ 10.39 & 42.56 $\pm$ 29.90 \\
Edge6 & 67.38 $\pm$ 8.92 & 89.16 $\pm$ 3.22 & 79.64 $\pm$ 6.55 & 90.21 $\pm$ 3.80 & 94.89 $\pm$ 0.74 & 20.70 $\pm$ 5.88 & 15.87 $\pm$ 17.10 & 35.47 $\pm$ 25.17 \\
Edge7 & 69.31 $\pm$ 9.42 & 91.62 $\pm$ 2.41 & 76.14 $\pm$ 8.61 & 90.89 $\pm$ 3.22 & 95.08 $\pm$ 0.74 & 45.07 $\pm$ 16.01 & 25.27 $\pm$ 26.69 & 33.21 $\pm$ 27.90 \\
Edge8 & 77.17 $\pm$ 3.08 & 90.52 $\pm$ 0.22 & 85.04 $\pm$ 1.73 & 92.93 $\pm$ 0.63 & 94.91 $\pm$ 0.78 & 40.87 $\pm$ 0.14 & 20.14 $\pm$ 5.76 & 51.55 $\pm$ 9.80 \\
\midrule
 & ant\_6\_b & ant\_4\_c & ant\_5\_c & ant\_6\_c & ant\_4\_d & ant\_5\_d & ant\_6\_d & \textbf{Average} \\
\midrule
MLP & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.76 $\pm$ 1.32 & 0.00 $\pm$ 0.00 & 0.20 $\pm$ 0.34 & 4.31 $\pm$ 7.02 & 0.78 $\pm$ 0.00 & 14.82 \% \\
AM  & 42.83 $\pm$ 21.22 & 4.78 $\pm$ 8.27 & 31.53 $\pm$ 15.00 & 11.01 $\pm$ 18.61 & 42.73 $\pm$ 11.70 & 45.57 $\pm$ 12.87 & 49.56 $\pm$ 9.27 & 58.87 \% \\
MM & 0.20 $\pm$ 0.34 & 11.80 $\pm$ 14.72 & 35.06 $\pm$ 21.47 & 41.31 $\pm$ 15.08 & 1.82 $\pm$ 3.16 & 7.51 $\pm$ 7.69 & 10.65 $\pm$ 8.91 & 35.27 \% \\
Edge1 & 51.30 $\pm$ 26.51 & 13.74 $\pm$ 8.08 & 19.33 $\pm$ 12.49 & 27.85 $\pm$ 21.10 & 6.85 $\pm$ 5.42 & 27.21 $\pm$ 22.37 & 30.69 $\pm$ 10.92 & 45.89 \% \\
Edge2 & 54.83 $\pm$ 15.26 & 1.48 $\pm$ 2.57 & 34.04 $\pm$ 20.87 & 47.93 $\pm$ 20.33 & 7.90 $\pm$ 8.03 & 39.97 $\pm$ 7.94 & 44.48 $\pm$ 13.13 & 47.70 \% \\
Edge3 & 55.68 $\pm$ 33.41 & 7.60 $\pm$ 12.71 & 23.23 $\pm$ 23.23 & 20.93 $\pm$ 25.23 & 9.49 $\pm$ 10.08 & 27.06 $\pm$ 15.52 & 24.42 $\pm$ 20.34 & 43.08 \% \\
Edge4 & 9.55 $\pm$ 14.78 & 0.96 $\pm$ 1.26 & 10.77 $\pm$ 11.04 & 9.48 $\pm$ 15.52 & 0.20 $\pm$ 0.34 & 27.13 $\pm$ 11.40 & 33.20 $\pm$ 11.55 & 41.12 \% \\
Edge5 & 49.64 $\pm$ 19.27 & 2.50 $\pm$ 4.33 & 15.61 $\pm$ 13.46 & 32.25 $\pm$ 22.92 & 3.82 $\pm$ 5.74 & 25.18 $\pm$ 17.97 & 23.25 $\pm$ 19.36 & 43.62 \% \\
Edge6 & 37.46 $\pm$ 29.62 & 8.34 $\pm$ 8.45 & 9.17 $\pm$ 13.69 & 9.43 $\pm$ 9.63 & 0.78 $\pm$ 0.55 & 30.35 $\pm$ 13.48 & 20.45 $\pm$ 18.28 & 40.62 \% \\
Edge7 & 35.57 $\pm$ 27.36 & 10.73 $\pm$ 9.03 & 5.71 $\pm$ 8.15 & 17.15 $\pm$ 19.40 & 6.23 $\pm$ 9.44 & 37.38 $\pm$ 13.00 & 44.58 $\pm$ 11.62 & 45.59 \% \\
Edge8 & 46.56 $\pm$ 4.05 & 0.39 $\pm$ 0.39 & 31.03 $\pm$ 27.98 & 14.28 $\pm$ 12.73 & 15.19 $\pm$ 15.19 & 46.37 $\pm$ 5.39 & 25.20 $\pm$ 25.20 & 48.81 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 14 morphologies in ant\_twisters (12k).}
\label{tab:ant_twisters_edge}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 66.43 $\pm$ 10.00 & 63.84 $\pm$ 15.94 & 72.54 $\pm$ 6.35 & 70.95 $\pm$ 6.38 & 68.44 \% \\
AM & 66.86 $\pm$ 9.14 & 86.40 $\pm$ 3.30 & 82.23 $\pm$ 6.53 & 64.57 $\pm$ 5.24 & 75.01 \% \\
AM - id & 73.12 $\pm$ 5.08 & 86.77 $\pm$ 4.36 & 82.94 $\pm$ 4.88 & 63.85 $\pm$ 1.31 & 76.67 \% \\
MM - m - jv - rp & 93.06 $\pm$ 2.17 & 95.80 $\pm$ 2.27 & 92.90 $\pm$ 2.03 & 71.93 $\pm$ 10.79 & 88.42 \% \\
MM - m - jv - rr & 72.95 $\pm$ 2.48 & 85.59 $\pm$ 1.16 & 84.61 $\pm$ 5.90 & 65.39 $\pm$ 3.17 & 77.14 \% \\
MM - m - jv & 90.48 $\pm$ 4.35 & 90.33 $\pm$ 6.04 & 92.98 $\pm$ 4.10 & 72.74 $\pm$ 7.90 & 86.63 \% \\
MM - m & 86.50 $\pm$ 4.34 & 92.13 $\pm$ 4.37 & 89.56 $\pm$ 4.44 & 69.12 $\pm$ 9.53 & 84.33 \% \\
MM & 75.58 $\pm$ 16.28 & 79.67 $\pm$ 4.91 & 87.88 $\pm$ 1.19 & 73.69 $\pm$ 5.78 & 79.20 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_b (12k).}
\label{tab:ant_twister_b_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 95.02 $\pm$ 2.02 & 45.19 $\pm$ 17.94 & 79.85 $\pm$ 5.33 & 54.41 $\pm$ 10.47 & 68.62 \% \\
AM & 98.07 $\pm$ 0.66 & 93.79 $\pm$ 1.02 & 96.90 $\pm$ 0.88 & 86.42 $\pm$ 2.49 & 93.80 \% \\
MM & 98.60 $\pm$ 0.88 & 89.15 $\pm$ 2.98 & 96.56 $\pm$ 0.59 & 87.45 $\pm$ 3.93 & 92.94 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_b (20k).}
\label{tab:ant_twister_b2_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 98.97 $\pm$ 0.35 & 70.89 $\pm$ 7.31 & 94.05 $\pm$ 1.01 & 84.56 $\pm$ 8.83 & 87.12 \% \\
AM & 99.95 $\pm$ 0.04 & 96.26 $\pm$ 0.83 & 99.47 $\pm$ 0.19 & 97.36 $\pm$ 0.59 & 98.26 \% \\
MM & 99.81 $\pm$ 0.16 & 96.01 $\pm$ 1.96 & 99.15 $\pm$ 0.24 & 97.62 $\pm$ 1.28 & 98.15 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_b (40k).}
\label{tab:ant_twister_b3_obs}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{1.0}{
\begin{tabular}{lcccc}
\toprule
 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 2.71 $\pm$ 1.92 & 5.63 $\pm$ 1.13 & 0.98 $\pm$ 0.65 & 3.11 \% \\
AM & 54.03 $\pm$ 5.41 & 66.22 $\pm$ 9.64 & 71.11 $\pm$ 5.73 & 63.79 \% \\
AM - id & 45.05 $\pm$ 9.11 & 64.56 $\pm$ 10.70 & 67.53 $\pm$ 15.62 & 59.05 \% \\
MM - m - jv - rp & 26.03 $\pm$ 8.72 & 40.10 $\pm$ 8.85 & 40.98 $\pm$ 11.66 & 35.71 \% \\
MM - m - jv - rr & 48.65 $\pm$ 6.90 & 66.14 $\pm$ 10.61 & 73.56 $\pm$ 8.96 & 62.78 \% \\
MM - m - jv & 26.91 $\pm$ 7.07 & 51.16 $\pm$ 2.99 & 52.04 $\pm$ 9.00 & 43.37 \% \\
MM - m & 18.49 $\pm$ 7.83 & 37.66 $\pm$ 10.03 & 36.04 $\pm$ 8.76 & 30.73 \% \\
MM & 0.59 $\pm$ 0.65 & 1.17 $\pm$ 0.87 & 0.98 $\pm$ 0.85 & 0.91 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_d (12k).}
% ant\_reach2\_handsup
\label{tab:ant_touch_handsup}
% \vskip -0.1in
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{1.0}{
\begin{tabular}{lcccc}
\toprule
 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 3.09 $\pm$ 2.10 & 1.95 $\pm$ 0.87 & 1.37 $\pm$ 0.65 & 2.13 \% \\
AM & 88.20 $\pm$ 0.77 & 95.27 $\pm$ 1.16 & 93.64 $\pm$ 2.14 & 92.37 \% \\
MM & 6.84 $\pm$ 9.67 & 14.63 $\pm$ 16.91 & 31.38 $\pm$ 4.34 & 17.61 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_d (20k).}
% ant\_reach2\_handsup
\label{tab:ant_touch_handsup2}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{1.0}{
\begin{tabular}{lcccc}
\toprule
 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 4.62 $\pm$ 2.31 & 10.63 $\pm$ 3.01 & 11.18 $\pm$ 2.40 & 8.81 \% \\
AM & 99.03 $\pm$ 0.22 & 99.39 $\pm$ 0.11 & 98.63 $\pm$ 0.48 & 99.02 \% \\
MM & 68.50 $\pm$ 7.41 & 79.68 $\pm$ 6.32 & 78.21 $\pm$ 1.11 & 75.46 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_d (40k).}
% ant\_reach2\_handsup
\label{tab:ant_touch_handsup3}
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{lcccccc}
\toprule
 & ant\_2 & ant\_3 & ant\_4 & ant\_5 & ant\_6 & \textbf{Average}  \\
\midrule
MLP & 70.89 $\pm$ 9.44 & 70.60 $\pm$ 11.10 & 48.77 $\pm$ 12.05 & 74.65 $\pm$ 7.68 & 97.08 $\pm$ 0.79 & 72.40 \% \\
AM & 66.72 $\pm$ 6.86 & 83.44 $\pm$ 3.48 & 74.72 $\pm$ 5.27 & 95.32 $\pm$ 0.49 & 96.35 $\pm$ 0.53 & 83.31 \% \\
AM - id & 78.85 $\pm$ 4.44 & 88.63 $\pm$ 2.37 & 82.70 $\pm$ 3.57 & 96.72 $\pm$ 0.50 & 98.49 $\pm$ 0.31 & 89.08 \% \\
MM - m - jv - rp & 73.67 $\pm$ 10.34 & 88.50 $\pm$ 1.46 & 83.38 $\pm$ 4.89 & 97.03 $\pm$ 1.01 & 97.21 $\pm$ 0.57 & 87.96 \% \\
MM - m - jv - rr & 79.16 $\pm$ 6.15 & 88.40 $\pm$ 0.88 & 77.80 $\pm$ 6.56 & 95.49 $\pm$ 1.16 & 97.92 $\pm$ 0.39 & 87.76 \% \\
MM - m - jv & 81.30 $\pm$ 4.46 & 86.77 $\pm$ 1.99 & 81.71 $\pm$ 6.05 & 98.09 $\pm$ 0.36 & 98.09 $\pm$ 0.20 & 89.19 \% \\
MM - m & 79.81 $\pm$ 3.62 & 83.77 $\pm$ 4.20 & 69.66 $\pm$ 6.07 & 96.45 $\pm$ 0.52 & 97.91 $\pm$ 0.43 & 85.52 \% \\
MM & 74.49 $\pm$ 3.39 & 84.62 $\pm$ 4.13 & 72.43 $\pm$ 5.48 & 94.63 $\pm$ 1.64 & 97.31 $\pm$ 0.45 & 84.70 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 4 morphologies in ant\_twister\_a (12k).}
\label{tab:ant_reach_handsup}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}



\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{lccccccc}
\toprule
 & centipede\_2 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average}  \\
\midrule
MLP & 48.34 $\pm$ 20.61 & 16.85 $\pm$ 10.59 & 12.21 $\pm$ 14.47 & 56.32 $\pm$ 17.45 & 75.63 $\pm$ 16.66 & 84.20 $\pm$ 3.95 & 48.93 \% \\
AM & 24.09 $\pm$ 18.49 & 23.70 $\pm$ 7.57 & 35.07 $\pm$ 18.20 & 60.30 $\pm$ 11.41 & 75.16 $\pm$ 6.03 & 83.56 $\pm$ 1.53 & 50.32 \% \\
AM - id  & 22.53 $\pm$ 7.66 & 32.85 $\pm$ 8.87 & 39.77 $\pm$ 25.28 & 79.59 $\pm$ 5.06 & 83.64 $\pm$ 10.67 & 84.70 $\pm$ 5.54 & 57.18 \% \\
MM - m - jv - rp & 18.27 $\pm$ 5.57 & 31.68 $\pm$ 11.81 & 47.35 $\pm$ 12.54 & 86.45 $\pm$ 4.88 & 82.70 $\pm$ 6.23 & 88.39 $\pm$ 2.16 & 59.14 \% \\
MM - m - jv - rr & 15.84 $\pm$ 6.31 & 26.86 $\pm$ 9.32 & 49.86 $\pm$ 11.82 & 85.92 $\pm$ 4.30 & 82.51 $\pm$ 5.70 & 87.97 $\pm$ 1.71 & 58.16 \% \\
MM - m - jv & 13.73 $\pm$ 2.26 & 24.67 $\pm$ 7.37 & 44.76 $\pm$ 7.21 & 80.38 $\pm$ 5.65 & 82.40 $\pm$ 3.15 & 87.16 $\pm$ 1.07 & 55.51 \% \\
MM - m  & 14.74 $\pm$ 5.92 & 18.17 $\pm$ 8.87 & 37.15 $\pm$ 12.54 & 86.39 $\pm$ 3.20 & 82.53 $\pm$ 2.33 & 90.24 $\pm$ 1.24 & 54.87 \% \\
MM  & 30.87 $\pm$ 16.86 & 31.36 $\pm$ 20.28 & 56.57 $\pm$ 9.93 & 82.49 $\pm$ 5.70 & 81.33 $\pm$ 3.31 & 85.51 $\pm$ 4.39 & 61.35 \% \\

\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in centipede\_twister\_a (12k).}
\label{tab:centipede_reach_handsup}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{lccccc}
\toprule
 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6 & \textbf{Average}  \\
\midrule
MLP & 14.50 $\pm$ 4.67 & 38.32 $\pm$ 7.86 & 38.23 $\pm$ 9.81 & 51.46 $\pm$ 12.22 & 35.63 \% \\
AM & 42.70 $\pm$ 12.98 & 74.97 $\pm$ 8.02 & 86.76 $\pm$ 3.87 & 86.09 $\pm$ 8.10 & 72.63 \% \\
AM - id  & 45.93 $\pm$ 12.43 & 55.76 $\pm$ 7.12 & 86.86 $\pm$ 2.79 & 89.25 $\pm$ 4.27 & 69.45 \% \\
MM - m - jv - rp  & 41.71 $\pm$ 9.05 & 58.23 $\pm$ 6.76 & 84.73 $\pm$ 2.41 & 86.42 $\pm$ 2.88 & 67.77 \% \\
MM - m - jv - rr & 49.05 $\pm$ 13.84 & 51.16 $\pm$ 6.40 & 83.82 $\pm$ 2.93 & 88.12 $\pm$ 1.14 & 68.04 \% \\
MM - m - jv & 41.92 $\pm$ 9.75 & 49.27 $\pm$ 7.54 & 87.15 $\pm$ 3.02 & 87.65 $\pm$ 4.07 & 66.50 \% \\
MM - m & 40.47 $\pm$ 5.02 & 46.19 $\pm$ 5.43 & 80.64 $\pm$ 6.82 & 84.35 $\pm$ 7.15 & 62.91 \% \\
MM  & 28.55 $\pm$ 12.93 & 42.00 $\pm$ 14.58 & 80.91 $\pm$ 2.37 & 87.06 $\pm$ 1.33 & 59.63 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in centipede\_twister\_b (12k).}
\label{tab:centipede_reach_handsup2}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{lcccccc}
\toprule
 & centipede\_3 & centipede\_4 & centipede\_5 & centipede\_6 & centipede\_7 & \textbf{Average}  \\
\midrule
MLP & 13.21 $\pm$ 1.58 & 7.34 $\pm$ 1.57 & 13.46 $\pm$ 3.71 & 11.38 $\pm$ 4.32 & 8.98 $\pm$ 2.25 & 10.87 \% \\
AM & 53.22 $\pm$ 10.70 & 81.61 $\pm$ 8.64 & 83.68 $\pm$ 5.92 & 78.75 $\pm$ 3.25 & 62.47 $\pm$ 5.86 & 71.94 \% \\
AM - id  & 64.40 $\pm$ 5.56 & 83.41 $\pm$ 3.11 & 87.93 $\pm$ 2.45 & 80.80 $\pm$ 1.38 & 65.31 $\pm$ 9.16 & 76.37 \% \\
MM - m - jv - rp & 70.93 $\pm$ 8.44 & 82.00 $\pm$ 2.62 & 87.97 $\pm$ 2.67 & 83.73 $\pm$ 3.81 & 66.64 $\pm$ 3.26 & 78.25 \% \\
MM - m - jv - rr  & 64.39 $\pm$ 11.95 & 85.29 $\pm$ 6.41 & 86.20 $\pm$ 4.03 & 83.67 $\pm$ 8.91 & 70.53 $\pm$ 5.38 & 78.02 \% \\
MM - m - jv  & 70.54 $\pm$ 6.91 & 80.74 $\pm$ 3.52 & 86.30 $\pm$ 4.16 & 82.60 $\pm$ 4.39 & 67.18 $\pm$ 7.58 & 77.47 \% \\
MM - m & 62.70 $\pm$ 5.63 & 78.13 $\pm$ 5.12 & 84.66 $\pm$ 0.89 & 79.23 $\pm$ 3.81 & 61.68 $\pm$ 5.82 & 73.28 \% \\
MM & 47.23 $\pm$ 10.69 & 35.66 $\pm$ 7.00 & 32.80 $\pm$ 9.64 & 36.92 $\pm$ 13.10 & 20.79 $\pm$ 8.03 & 34.68 \% \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{The average success rate over 5 morphologies in centipede\_twister\_d (12k).}
\label{tab:centipede_touch_handsup}
% AM - id == MM - m - jv - rp - rr
% \vskip -0.1in
\end{table*}

==> data_entry_wrapfig.tex <==
\begin{wrapfigure}{R}[0pt]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/data_entry2.pdf}
\vspace{-5pt}
\caption{
The average normalized final distance with different size of datasets (left) and morphology-task combinations (right). See \autoref{sec:embodiment_bench_details} for entry separation.
These results suggest that the performance can get better when we increase the number of datasets, and can surpass the degradation of the performance when we increase the number of entries.
}
\label{fig:data_entry}
\end{wrapfigure}

==> embodiment_bench_figure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.825\linewidth]{fig/embodiment_bench.pdf}
    \vspace{-5pt}
    \caption{The overview of Embodiment Bench, which can procedurally generate both various morphologies and tasks with minimal blueprints.
    Embodiment Bench can not only construct the agents with different number of limbs, but also randomize missing limbs and size or mass of limbs.
    We could also design the tasks with parameterized goal distributions.
    It also supports to import custom complex agents such as unimals~\citep{gupta2022metamorph}.
    }
    \label{fig:embodiment_bench}
\end{figure*}


==> embodiment_bench_table.tex <==
\begin{table*}[htb]
\begin{center}
\begin{small}
\scalebox{0.85}{
\begin{tabular}{l|ccc}
\toprule
\textbf{Benchmark} & \textbf{Multi-Task} & \textbf{Multi-Morphology} & \textbf{Scalability} \\
\midrule
MuJoCo \& DM Control & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} \\
Meta-World~\citep{yu2019meta} & \textcolor{green}{\CheckmarkBold} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} \\
\citet{huang2020policy} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\CheckmarkBold} &  \textcolor{red}{\XSolidBrush}\\
\citet{gupta2022metamorph} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} \\
\textbf{\proposedbench (Ours)} & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{
Comparison among relevant RL benchmarks for continuous control. We review whether they are suitable to evaluate morphology-task generalization, in terms of (1) multi-task (task coverage), (2) multi-morphology (morphology coverage), and (3) scalability.
MuJoCo~\citep{todorov2012mujoco} and DM Control~\citep{tassa2018deepmind} only have a single morphology for a single task. While other existing works~\citep{yu2019meta,huang2020policy,gupta2022metamorph} partially cover task or morphology diversity with some sort of scalability, they do not satisfy all criteria.
We develop \proposedbench, which has multiple tasks and morphologies with functionalities for procedural generation and minimal blueprints.
}
\label{tab:embodiment_bench}
\vskip -0.1in
\end{table*}


==> local_observations_old.tex <==
\section{Representation Selection: Local Observations}
\label{sec:local_obs_details}

In this section, we explore the set of node features that is most suitable for behavior distillation in multi-morphology-multi-task settings, and provide the design principle of node features.
Previous morphology-agnostic studies have worked on searching network architectures that could efficiently process the encoded morphological graph, such as GNN~\citep{wang2018nervenet,blake2021snowflake}, GNN for tree structure~\citep{huang2020policy}, and various Transformers~\citep{kurin2020my,gupta2022metamorph,br2022anymorph,hong2022structureaware}.
However, it is still unclear what kind of observations in the system could contribute to morphology-task generalization as the local features for each node of \proposedrep{}.
It could be valuable to identify how each feature contributes to goal-reaching or generalization and which sets of node features perform best.

There are a lot of observable candidates per module in the agent's system, such as Cartesian position (\textbf{p}), Cartesian velocity (\textbf{v)}, quotation (\textbf{q}), angular velocity (\textbf{a}), joint angle (\textbf{ja}), joint range (\textbf{jr}), limb id (\textbf{id}), joint velocity (\textbf{jv}), relative position (\textbf{rp}), relative rotation (\textbf{rr}), and morphological information (\textbf{m}).
Morphological information contains module's shape, mass, inertia, actuator's gear, and dof-index, etc.
To shed light on the importance of the local representation per module, we execute an extensive ablation of node feature selections and prepossessing.
In prior works, \citet{huang2020policy} and the following~\citep{kurin2020my,hong2022structureaware} used \{\textbf{p}, \textbf{v}, \textbf{q}, \textbf{a}, \textbf{ja}, \textbf{jr}, \textbf{id}\} and \citet{gupta2022metamorph} used \{\textbf{p}, \textbf{v}, \textbf{q}, \textbf{a}, \textbf{ja}, \textbf{jr}, \textbf{jv}, \textbf{rp}, \textbf{rr}, \textbf{m}\}.
Considering the intersection of those, we define \{\textbf{p}, \textbf{v}, \textbf{q}, \textbf{a}, \textbf{ja}, \textbf{jr}\} as \texttt{base\_set} and test the combination to other observations (\textbf{jv}, \textbf{id}, \textbf{rp}, \textbf{rr}, \textbf{m}).


We prepare In-Distribution division in~\autoref{tab:zs_morph_entry} and evaluate in-distribution generalization with \proposedshort{} representation.
\autoref{tab:node_feat} shows that, while some additional features (\textbf{id}, \textbf{rp}, \textbf{m}) contribute to improving the goal-reaching performance, the most effective feature seems morphological information (\textbf{m}).
These results suggest \texttt{base\_set} contains sufficient features for control, and raw morphological properties (\textbf{m}) serves better task specification than manually-encoded information such as limb id (\textbf{id}).
The key observations are; (1) morphological information is critical for morphology-task generalization, and (2) extra observation might disrupt the goal-reaching performances, such as relative rotation between parent and child node (\textbf{rr}).
Throughout the paper, we use \texttt{base\_set-m} for node features of \proposedrep{} representation.

\begin{table*}[ht]
\begin{center}
\begin{small}
\scalebox{1.}{
\begin{tabular}{l|ccccc|l}
\toprule
Node features & +\textbf{jv} & +\textbf{id} & +\textbf{rp} & +\textbf{rr} & +\textbf{m} & \textbf{Average Dist.} \\
\midrule
\texttt{base\_set} & & & & & & 0.4330 $\pm$ 0.02 \\
\texttt{base\_set-id} & & \textcolor{green}{\CheckmarkBold} & & & & 0.4090 $\pm$ 0.02 \\
\texttt{base\_set-rp} & & & \textcolor{green}{\CheckmarkBold} & & & 0.3820 $\pm$ 0.01 \\
\texttt{base\_set-rr} & &  &  & \textcolor{green}{\CheckmarkBold} & & 0.4543 $\pm$ 0.01 \\
\texttt{base\_set-m} & &  &  &  & \textcolor{green}{\CheckmarkBold} & \textbf{0.3128 $\pm$ 0.02}\\
\texttt{base\_set-rp-rr} & &  & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} & & 0.3869 $\pm$ 0.01 \\
\texttt{base\_set-jv-rp-rr} & \textcolor{green}{\CheckmarkBold} &  & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} & & 0.4000 $\pm$ 0.01 \\
\texttt{base\_set-jv-rp-rr-m} & \textcolor{green}{\CheckmarkBold} &  & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} & \textcolor{green}{\CheckmarkBold} & 0.3323 $\pm$ 0.01\\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\caption{
Combination of control-oriented node features. We compare the combination of Cartesian position (\textbf{p}), Cartesian velocity (\textbf{v)}, quotation (\textbf{q}), angular velocity (\textbf{a}), joint angle (\textbf{ja}), joint range (\textbf{jr}), limb id (\textbf{id}), joint velocity (\textbf{jv}), relative position (\textbf{rp}), relative rotation (\textbf{rr}), and morphological information (\textbf{m}).
\texttt{base\_set} is composed of \{\textbf{p}, \textbf{v}, \textbf{q}, \textbf{a}, \textbf{ja}, \textbf{jr}\}. 
In prior works, \citet{huang2020policy,kurin2020my,hong2022structureaware} used \texttt{base\_set-id} and \citet{gupta2022metamorph} used \texttt{base\_set-jv-rp-rr-m}.
While some additional features (\textbf{id}, \textbf{rp}, \textbf{m}) contribute to improving the goal-reaching performance, the most effective feature seems morphological information (\textbf{m}).
These results suggest \texttt{base\_set} contains sufficient features for control, and raw morphological properties (\textbf{m}) serves better task specification than manually-encoded information such as limb id (\textbf{id}).
}
% \label{tab:node_feat}
% \vskip -0.1in
\end{table*}

